Query-Reduction Networks for Question Answering

In this paper, we study the problem of question answering when reasoning over multiple facts is required. We propose Query-Reduction Network (QRN), a variant of Recurrent Neural Network (RNN) that effectively handles both short-term (local) and long-term (global) sequential dependencies to reason over multiple facts. QRN considers the context sentences as a sequence of state-changing triggers, and reduces the original query to a more informed query as it observes each trigger (context sentence) through time. Our experiments show that QRN produces the state-of-the-art results in bAbI QA and dialog tasks, and in a real goal-oriented dialog dataset. In addition, QRN formulation allows parallelization on RNN's time axis, saving an order of magnitude in time complexity for training and inference.

==> 06-sent.tex <==

\subsection{Data}
We also report QRN's performance on Stanford Sentiment Treebank~\citep{socher2013recursive}, a popular dataset for sentiment classification.
We train and test our QRN model on the binary classification task, which consists of 6920 training, 872 development, and 1820 test examples.

\subsection{Model Details}
\paragraph{Input and Output Module.} 
In sentiment analysis, there is only one sentence (instead of multiple facts in a story) and there is no explicit question.
We instead let each word of the sentence occupy single fact slot ${\bf x}_t$ in QRN, and fix the question vector ${\bf q}$ to be a constant vector of $0.1$. MemNNs
The embedding of each word is obtained via GloVe~\citep{pennington2014glove}, pre-trained on 840B Common Crawl corpora (we did not finetune).
This gives us a $300$-dimensional vector for each word.
Single $\tanh$ perceptron layer is used to transform each word vector to the QRN's hidden state size, $d$.
For output module, we use a binary single layer softmax classifier to map $\hat{y}$ to $\{positive, negative\}$ labels.

\paragraph{Training.}
Hidden state size ($d$) is set to 100 and the batch size is $128$.
We stack two layers of QRNs.
All weights are initialized using techniques from~\citet{glorot2010understanding}.
Forget bias is $2.5$  for update gates ($z^k_t$), and L2 weight decay of $0.001$ is used for all weights.
In addition, we use dropout~\citep{srivastava2014dropout} on the inputs of Equation~\ref{eq:h}.
The model is trained with AdaGrad~\citep{duchi2011adaptive} with initial learning rate of $0.5$, for 50 epochs.
We repeated the training procedure with new random weight initialization for 30 times and reported the test data result with the lowest development data loss.

\subsection{Results.}
Figure~\ref{fig:sst} shows QRN results compared against state-of-the-art methods.
% It is important to note that all of the baselines is RNN- or CNN-based architecture, while ours does not use either of those.
The result first confirms that our model can effectively incorporate inter-word dependencies without putting perceptron layers across the time axis, as QRN outperforms two strong RNN-based baselines, MV-RNN and RNTN~\citep{socher2013recursive}.
However, QRN is still short of recent state-of-the-art results, including DMN. To an extent, this is not a surprising result since inter-dependency between words is much higher than that between sentences.
In particular,  QRN is targeted for weak, long-term interdependent data; we cannot take the full advantage of QRN  in this dataset. On the other hand, 
QRN is simpler than the baseline models and can be parallelized across time. 

%As a future direction, we plan to explore combining RNN architecture with our model, though this would sacrifice the parallelization.


\begin{figure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|ccccc|c|}
\hline
& MV-RNN~\citep{socher2013recursive} & RNTN~\citep{socher2013recursive} & DCNN~\citep{DCNN} & CNN-MC~\citep{CNN-MC} & DMN~\citep{DMN} & QRN \\
\hline
Accuracy ($\%$) & 82.9 & 85.4 & 86.8 & 88.1 & 88.6 & 85.8 \\
\hline
\end{tabular}
}
\end{center}
\caption{Results on binary sentiment classification of Stanford Sentiment Treebank~\citep{socher2013recursive}}
\label{fig:sst}
\end{figure}

==> ICLR 2017 QRN/01-intro.tex <==


%Machine comprehension (MC) is the task of obtaining the answer to a natural language question given a sequence of natural language sentences (story)~\citep{MCTest,squad}.
%We are particularly interested in the task of \emph{end-to-end} MC, where 
%(1) external language resources, such as lexicon or dependency parser, are not provided, and 
%(2) the only supervision during training is the answer to the question.
%This task becomes particularly challenging when answering a question requires logical reasoning by selecting relevant facts from a large pool of sentences and combining them in a correct order to answer the question.
In this paper, we address the problem of  question answering (QA) when reasoning over multiple facts is required. 
For example, consider we know that \texttt{Frogs eat insects} and \texttt{Flies are insects}. 
Then answering \texttt{Do frogs eat flies?} requires reasoning over both of the above facts. Question answering, more specifically context-based QA, has been extensively studied in machine comprehension tasks~\citep{MCTest,hermann2015teaching,hill2015goldilocks,squad}. However, most of the datasets are primarily focused on lexical and syntactic understanding, and hardly concentrate on inference over multiple facts. 
Recently, several datasets aimed for testing multi-hop reasoning have emerged; among them are story-based QA~\citep{babi} and the dialog task~\citep{bordes2016learning}.

Recurrent Neural Network (RNN) and its variants, such as Long Short-Term Memory (LSTM)~\citep{lstm} and Gated Recurrent Unit (GRU)~\citep{GRU}, are popular choices for modeling natural language. However, when used for multi-hop reasoning in question answering, purely RNN-based models have shown to perform poorly~\citep{babi}. This is largely due to the fact that RNN's internal memory is inherently unstable over a long term. For this reason, most recent approaches in the literature have mainly relied on global attention mechanism and shared external memory~\citep{memN2N,NR,DMN+,graves2016hybrid}.
The attention mechanism allows these models to focus on a single sentence in each layer.
They can sequentially read multiple relevant sentences from the memory with multiple layers to perform multi-hop reasoning. However, one major drawback of these standard attention mechanisms is that they are insensitive to the time step (memory address) of the sentences when accessing them.
% That is, it cannot differentiate between the same sentences at different time steps even though they can have different meanings.
% End-to-end Memory Network~\citep{memN2N} attempts to resolve this problem by adding time-dependent variable to the sentence representation at each time step (address) of the memory.
% Dynamic Memory Network~\citep{DMN,DMN+} combines RNN and attention mechanism together to incorporate time dependency into the model.

Our proposed model, Query-Reduction Network\footnote{Code is publicly available at: \url{seominjoon.github.io/qrn/}}(QRN), is a single recurrent unit that addresses the long-term dependency problem of most RNN-based models by simplifying the recurrent update, while taking the advantage of RNN's capability to model sequential data (Figure~\ref{fig:model}).
QRN considers the context sentences as a sequence of state-changing triggers, and transforms (\emph{reduces}) the original query to a more informed query as it observes each trigger through time. 
For instance in Figure~\ref{fig:qrn_ex}, 
the original question, \texttt{Where is the apple?}, cannot be directly answered by any single sentence from the story. After observing the first sentence, \texttt{Sandra got the apple there}, QRN transforms the original question to a reduced query \texttt{Where is Sandra?}, which is presumably easier to answer than the original question given the context provided by the first sentence.\footnote{This mechanism is akin to logic regression in situation calculus~\citep{reiter}.}
% While previous work~\citep{memNet,memN2N,NR,DMN,DMN+} can be also viewed as performing query regression through multiple layers,
Unlike RNN-based models, QRN's candidate state ($\tilde{\bf h}_t$ in Figure~\ref{fig:unit}) does not depend on the previous hidden state (${\bf h}_{t-1}$). 
Compared to memory-based approaches~\citep{memNet,memN2N,NR,DMN,DMN+}, QRN can better encodes \emph{locality} information because  it does not use a global memory access controller (circle nodes in Figure~\ref{fig:models}), and the query updates are performed locally.


In short, the main contribution of QRN is threefold. 
First, QRN is a simple variant of RNN that {\it reduces} the query given the context sentences in a differentiable manner.
Second, QRN is situated between the attention mechanism and RNN, effectively handling time dependency and long-term dependency problems of each technique, respectively. 
Hence it is well-suited for sequential data with both local and global interactions (note that QRN is \emph{not} the replacement of RNN, which is arguably better for modeling complex local interactions).
Third, unlike most RNN-based models, QRN can be parallelized over time by computing candidate reduced queries ($\tilde{\bf h}_t$) directly from local input queries (${\bf q}_t$) and context sentence vectors (${\bf x}_t$).
In fact, the parallelizability of QRN implies that QRN does not suffer from the vanishing gradient problem of RNN, hence effectively addressing the long-term dependency.
We experimentally demonstrate these contributions by achieving the state-of-the-art results on story-based QA and interactive dialog datasets.
% On the other hand, in QRN, candidate local queries (${\tilde {\bf h}}_t$) and the gates ($z_t,r_t$) are computed without previous hidden states, and ${\bf h}_t$ can be directly obtained from them.

\begin{figure}[t]
\centering
\begin{subfigure}[htbp]{0.242\textwidth}
\includegraphics[width=\textwidth]{figures/unit.pdf}
\caption{  QRN unit }
\label{fig:unit}
\end{subfigure}
\begin{subfigure}[htbp]{0.565\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/qrn_ex.pdf}
\caption{2-layer QRN}
\label{fig:qrn_ex}
\end{subfigure}
\begin{subfigure}[htbp]{0.143\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/overview.pdf}
\caption{Overview}
\label{fig:overview}
\end{subfigure}
\caption{\small (\ref{fig:unit}) QRN unit, (\ref{fig:qrn_ex})  2-layer QRN on 5-sentence story, and (\ref{fig:overview}) entire QA system (QRN and input / output modules). 
    ${\bm x}, {\bm q}, \hat{\bm y}$ are the story, question and predicted answer in natural language, respectively.
    ${\bf x}=\langle {\bf x}_1, \ldots , {\bf x}_T \rangle, {\bf q}, \hat{\bf y}$ are their corresponding vector representations (upright font).
    $\alpha$ and $\rho$ are update gate and reduce functions, respectively.
    ${\hat {\bf y}}$ is  assigned to be ${\bf h}^2_5$, the local query at the last time step in the last layer.
    Also, red-colored text is the inferred meanings of the vectors (see `Interpretations' of Section~\ref{subsec:results}). }
\label{fig:model}
\end{figure}


%In our experiments, we show that QRN outperforms the state of the art in bAbI 1k dataset~\citep{babi}, a synthetic story-based QA dataset that has recently become an important standard in the literature.
%We also explored if QRN can be a reasonable replacement for RNN-based models; we show that QRN outperforms LSTM in sentiment classification~\citep{socher2013recursive}, even though QRN is simpler\footnote{something here} and about 50 times faster to train and test than LSTM.



% Existing models in the literature have naturally focused on accumulating and summarizing information across the entire story in each layer to guide the attention in the next layer. However, encoding inter-dependencies among a large set of facts into a single vector imposes a challenge. While most of these methods have focused on progressing the state of the story only through layers, we propose to perform {\it logical regression} from the question through both time and layers. In this paper, we introduce Query-Regression Networks (QRNs) that \textit{regress} the query to a former or less developed state by observing facts. This is akin to logical regression mechanism in situation calculus that reasons about a query in a situation by regressing it back to the previous situation given the current action~\citep{reiter}. 

% Query-Regression Networks are inspired by recent advances in using memory, attention, and end-to-end trainable models, but update the question at each step. This allows QRNs to have fewer parameters compared to state of the art models. QRNs  can answer questions after each time step and  encode locality information because they do not require to accumulate all the information before passing it to the next layer.  Moreover, QRNs can be parallelized unlike approaches that use recurrent models; the question updates  only depend on the question at the previous state and the original facts can be decomposed across time steps.   Additionally, QRNs modify the typical attention mechanisms with a sigmoid layer that allows for attending on multiple facts at one pass. Finally, QRNs modify the sequential updates by using reset gates that allow the model to switch the attention. Figure~\ref{fig:model} depicts the architecture of QRNs. 

% Our experimental evaluations show that QRN outperform state-of-the-art comprehension systems when training data is limited, and are on-par with them when more training data exists. In addition, QRNs provide interpretable intermediate representations for question updates (Figure~\ref{fig:model}). Finally, we show that QRNs are general enough that can also be applied to other NLP tasks such as sentiment analysis.






%Often times the facts are time-sensitive; that is, the semantics of the story is dependent on the order of the sentences.
%For instance, suppose we are given a story of three sentences:``Mary went to the office'', ``Mary put down a football'', and ``Mary went to the bathroom''.
%Changing the order of the sentences clearly alters the final location of the football.



%\note{Interesting example, but we should move it:}
%For instance, Suppose ``John picked up ball'' at time 1, ``John dropped the ball'' at time 5, and ``John went to bathroom'' at time 10.
%Suppose the question is ``Where is the ball?''.
%After the system attending on fact 1, then the new question will be ``Where is John?''. However, the answer shouldn't be coming from fact 10, because he already dropped the ball at time 5.


==> ICLR 2017 QRN/02-model.tex <==

In story-based QA (or dialog dataset), the input is the \emph{context} as a sequence of sentences (story or past conversations) and a \emph{question} in natural language (equivalent to the user's last utterance in the dialog). 
The output is the predicted answer to the question in natural language (the system's next utterance in the dialog).
The only supervision provided during training is the answer to the question. 

% \vspace{-.4cm}

%\paragraph{Notation.} We use lowercase, boldface letters to denote column vectors (e.g. ${\bf x}$), and uppercase, boldface letters (e.g. ${\bf W}$) to denote matrices.
%Non-boldface italic letters denote scalar values (e.g. $t,T,d$), and
%boldface italic letters denote non-numerical objects such as a sentence (e.g. $\bm{x}$). $\top$ is used to denote vector or matrix transpose.
%Scalar and vector functions will be denoted by non-boldface and boldface lowercase Greek letters (e.g. $\alpha$, ${\bm \rho}$), respectively.
%$[;]$ is the concatenation of vectors across row, and $[,]$ is the concatenation of vectors across column.
%$\langle , \rangle$ denotes a sequence.
%A subscript denotes time step ($t$) in the story, and a superscript denotes the layer index ($k$) of the network.
%A superscript with parenthesis (e.g. ${\bf W}^{(z)}$, ${\bf W}^{({\bf h})}$) indicates that the weight matrix or vector is used to compute the value in the parenthesis (e.g. $z$, ${\bf h}$).
% ``Question'' refers to the original question, which is a sequence of word symbols. 
% ``Query'' refers to any abstract transformed form of the original question, including the question itself.

In this paper we particularly focus on end-to-end solutions, i.e.,  the only supervision comes from questions and answers, and we restrain from using manually defined rules or external language resources, such as lexicon or dependency parser. %\note{Do we have anything to say why we decided not to use external language resources? Or this is too obvious to the ICLR crowd? I think ICLR crowd will understand..}.
Let $\langle \bm{x}_1, \ldots, \bm{x}_T\rangle$ denote the sequence of sentences,  where $T$ is the number of sentences in the story, and let $\bm{q}$ denote the question. 
Let $\hat{\bm{y}}$ denote the predicted answer, and ${\bm{y}}$ denote the true answer.
Our proposed system for end-to-end QA task is divided into three modules (Figure~\ref{fig:overview}): input module, QRN layers, and output module.

\paragraph{Input module.} 
Input module maps each sentence $\bm{x}_t$ and the question $\bm{q}$ to $d$-dimensional vector space, ${\bf x}_t \in \mathbb{R}^d$ and ${\bf q}_t \in \mathbb{R}^d$.
We adopt a previous solution for the input module (details in Section~\ref{sec:qa}).

\paragraph{QRN layers.} 
QRN layers use the sentence vectors and the question vector from the input module to obtain the predicted answer in vector space, $\hat{\bf y} \in \mathbb{R}^d$. 
A QRN layer refers to the recurrent application of a QRN unit, which can be considered as a variant of RNN with two inputs, two outputs, and a  hidden state (reduced query), all of which operate in vector space.
The details of the QRN module is explained throughout this section (\ref{sec:model}, \ref{sec:var}).

\paragraph{Output module.}
Output module maps $\hat{\bf y}$ obtained from QRN to a natural language answer $\hat{\bm y}$. 
Similar to the input module, we adopt a standard solution for the output module (details in Section~\ref{sec:qa}).


We first formally define the base model of a QRN unit, and then we explain how we connect the input and output modules to it (Section~\ref{sec:model}).
We also present a few extensions to the network that can improve QRN's performance (Section~\ref{sec:var}).
Finally, we show that QRN can be parallelized over time, giving computational advantage over most RNN-based models by one order of magnitude (Section~\ref{sec:par}).

%\paragraph{Input Module.} This is an embedding function that maps each sentence $\bm{x}_t$ and the question $\bm{q}$ into a $d$-dimensional vector space.  
%Let $\langle {\bf m}_1, \dots, {\bf m}_T \rangle$ represent the embeddings of $T$ sentences of the story in $d$-dimensional vector space, and let ${\bf u} \in \mathbb{R}^d$ represent the embedding of the question $\bm{q}$. 
%\paragraph{Query Update Module.} 
%For each fact $m_t$, this module transfers the original question vector ${\bf u}$ into a new query vector. 
%Intuitively, the answer to the new query is equivalent to the answer to the original question, but the new query is easier to answer than the original question.
%For instance, consider the story $\langle  \bm{x}_1:\text{``John picked up the football.''}\rangle$ and the initial query vector  ${\bf u}$ that encodes ``Where is football?'' 
%Then the new query vector should encode ``Where is John?''. 
%The query update module uses attention mechanisms, reset gates, and incremental updates through multiple layers.  
%The details of how the updates are modeled is described in Section~\ref{sec:model}. 
%\paragraph{Answering Module.} At each time step $t$, the model answers the new updated query at that time. 
%We  obtain the answer $\hat{{\bf y}}_t \in \mathbb{R}^V$  as a one-hot encoding of vocabulary dictionary of size $V$.
% The final answer $\hat{{\bf y}}$ is the $\hat{{\bf y}}_T$. 


%Although most of the times questions ask about the final state ($t = T$), 
%some questions are interested in intermediate states.
%For instance, consider a question ``Where was football before bedroom?'' and a two-fact story ``John took the football to office. He then took it to the bedroom''.
%Here, the question is interested in where the football was at $t=1$, not the final state $t=2$.
%So, the answering module first finds the answer to the partial question ``Where was football?'' for each fact (``office'' and ``bedroom''),
%and then the selection module selects $t=1$, which is ``before the bedroom'', yielding the answer ``office''.

\subsection{QRN Unit}\label{sec:model}
%We first  define the networks on the first layer ($l=1$) of $u$.
%By its recursive definition, stacking several layers of $u$ will be straightforward.
As an RNN-based model, QRN is a single recurrent unit that updates its hidden state (reduced query) through time and layers. Figure~\ref{fig:unit} depicts the schematic structure of a QRN unit, and Figure~\ref{fig:qrn_ex} demonstrates how layers are stacked.
A QRN unit accepts two inputs (\emph{local} query vector ${\bf q}_t \in \mathbb{R}^d$ and sentence vector ${\bf x}_t \in \mathbb{R}^d$), and two outputs (reduced query vector ${\bf h}_t \in \mathbb{R}^d$, which is similar to the hidden state in RNN, and the sentence vector ${\bf x}_t$ from the input without modification).
The local query vector is not necessarily identical to the original query (question) vector ${\bf q}$.
In order to compute the outputs, we use \emph{update gate} function $\alpha: \mathbb{R}^d \times \mathbb{R}^d \rightarrow [0, 1]$ and \emph{reduce} function $\bm{\rho}: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}^d$. 
Intuitively, the update gate function measures the relevance between the sentence and the local query and is used to update the hidden state. 
The reduce function transforms the local query input to a candidate state which is a new reduced (easier) query given the sentence.
The outputs are calculated with the following equations:
\begin{eqnarray}\label{eq:z}
&& z_t= \alpha({\bf x}_t, {\bf q}_t) = \sigma({\bf W}^{(z)} ({\bf x}_t \circ {\bf q}_t) + b^{(z)})\\
%\end{equation}
%\begin{equation}\label{eq:ht}
&&{\tilde {\bf h}}_t = {\bm \rho}({\bf x}_t, {\bf q}_t) = \tanh({\bf W}^{({\bf h})}[{\bf x}_t; {\bf q}_t] + {\bf b}^{({\bf h})}) \label{eq:ht}\\
%\end{equation}
%\begin{equation}\label{eq:h}
&&{\bf h}_t = z_t {\tilde {\bf h}}_t + (1 - z_t) {\bf h}_{t-1}\label{eq:h}
\end{eqnarray}
where $z_t$ is the scalar update gate, ${\tilde {\bf h}}_t$ is the candidate reduced query, and ${\bf h}_t$ is the final reduced query at time step $t$,
$\sigma(\cdot)$ is sigmoid activation, $\tanh(\cdot)$ is hyperboolic tangent activation (applied element-wise),
${\bf W}^{(z)} \in \mathbb{R}^{1 \times d}$, ${\bf W}^{({\bf h})} \in \mathbb{R}^{d \times 2d}$ are weight matrices, 
$b^{(z)} \in \mathbb{R}$, ${\bf b}^{({\bf h})} \in \mathbb{R}^d$ are bias terms,
$\circ$ is element-wise vector multiplication, and $[;]$ is vector concatenation along the row.
As a base case, ${\bf h}_0 = {\bf 0}$.
Here we have explicitly defined $\alpha$ and ${\bm \rho}$,
but they can be any reasonable differentiable functions.

The update gate is similar to the global attention mechanism~\citep{memN2N,DMN+} in that it measures the similarity between the sentence (a memory slot) and the query.
However, a significant difference is that the update gate is computed using sigmoid ($\sigma$) function on the current memory slot only (hence internally embedded within the unit), whereas the global attention is computed using $\mathrm{softmax}$ function over the entire memory (hence globally defined).
The update gate can be rather considered as \emph{local sigmoid} attention.

\paragraph{Stacking layers} We just showed the single-layer case of QRN, but QRN with multiple layers is able to perform reasoning over multiple facts more effectively, as shown in the example of Figure~\ref{fig:qrn_ex}.
In order to stack several layers of QRN, the outputs of the current layer are used as the inputs to the next layer. 
That is, using superscript $k$ to denote the current layer's index (assuming $1$-based indexing), we let 
${\bf q}^{k+1}_t = {\bf h}^k_t$.
Note that ${\bf x}_t$ is passed to the next layer without any modification, so we do not put a layer index on it.

\paragraph{Bi-direction.}
So far we have assumed that QRN only needs to look at past sentences, whereas
often times, query answers can depend on future sentences.
For instance, consider a sentence ``John dropped the football.'' at time $t$.
Then, even if there is no mention about the ``football'' in the past (at time $i < t$), 
it can be implied that ``John'' has the ``football'' at the current time $t$. 
In order to incorporate the future dependency, we obtain $\overrightarrow{{\bf h}}_t$ and $\overleftarrow{{\bf h}}_t$ in both forward and backward directions, respectively, using Equation~\ref{eq:h}. We then  add them together to get ${\bf q}_t$ for the next layer. That is,
\begin{equation}
{\bf q}^{k+1}_t = \overrightarrow{{\bf h}}^k_t + \overleftarrow{{\bf h}}^k_t
\end{equation}
for layer indices $1 \leq k \leq K-1$.
Note that  the variables ${\bf W}^{(z)}, b^{(z)}, {\bf W}^{({\bf h})}, {\bf b}^{({\bf h})}$ are shared between the two directions.

\paragraph{Connecting input and output modules.}
Figure~\ref{fig:overview} depicts how QRN is connected with the input and output modules. 
In the first layer of QRN, ${\bf q}^1_t = {\bf q}$ for all $t$, where ${\bf q}$ is obtained from the input module by processing the natural language question input ${\bm q}$.
${\bf x}_t$ is also obtained from ${\bm x}_t$ by the same input module.
The output at the last time step in the last layer is passed to the output module.
That is, ${\hat {\bf y}} = {\bf h}^K_t$ where $K$ represent the number of layers in the network.
Then the output module gives the predicted answer ${\hat {\bm y}}$ in natural language.

%QRN consists of several layers of query-regression, and its components are recursively defined across time ($t$) and layers ($l$).
%Let ${\bf u}_t^0$ represent the question input to the first layer ($l=1$) at time $t$ ($\forall t.{\bf u}_t^0 = {\bf u}$).
%This serves as the base case for the recursive definitions to be demonstrated below.

%We first define attention gate $a^l_t$ at each time step $t$, which indicates the importance of the fact at that time, ${\bf m}_t$, given the query vector from the previous layer, ${\bf u}^{l-1}_t$.
%Therefore, in the first layer ($l=1$), the query vector from the previous layer corresponds to the original query vector, ${\bf u}$, as a base case. 
%$a^l_t$ is computed by
%\begin{equation}\label{eqn:a}
%    a^l_t = \sigma({\bf W}^{(a)} ({\bf u}^{l-1}_t \circ {\bf m}_t) + b^{(a)})
%\end{equation}
%where $\sigma$ is a sigmoid activation function,
%${\bf W}^{(a)} \in \mathbb{R}^{1 \times d}$ is a weight matrix, 
%$b^{(a)} \in \mathbb{R}$ is a scalar bias,
%and $\circ$ is element-wise vector multiplication.
%Note that $\circ$ can be replaced with an arbitrary function that encodes similarity %information between two vectors.
%It is important to note that our definition of attention is different from that of previous %work~\citep{memN2N,DMN+,DMN}, as we do not use softmax  to select a single fact.
%Hence it is possible to have high attention ($a^l_t$ being close to $1$) on several facts at different time steps, and clearly $\sum_t a^l_t = {\bf 1}$ is not guaranteed.

% It is sometimes useful to enforce all rows of $W^{(a)}$ and $b^{(a)}$ to be identical, which means all elements of $a^l_t$ will be equal.
% Then $a^l_t$ can be considered as a scalar value.

%We also define reset gate $r^l_t$ to nullify the query vector from previous time step ($t-1$). 
%For example, consider the story $\langle \bm{x}_1=\text{``Mary moved to the garden''}, \bm{x}_2=\text{``Mary dropped the football''}, \bm{x}_3=\text{``Mary went to the kitchen.''}\rangle$. 
%For the question  $\bm{q}:$``Where is football?'', The location of ``Mary'' becomes no more relevant to the question after $\bm{x}_2$.
%Intuitively, the reset gate {\it resets} the information that ``football'' is contained by ``Mary'' after she drops it. 
%We  compute reset gate $r^l_t$  by
%\begin{equation}\label{eqn:r}
%    r^l_t = \sigma({\bf W}^{(r)} ({\bf u}^{l-1}_t \circ {\bf m}_t) + b^{(r)})
%\end{equation}
%Where ${\bf W}^{(r)} \in \mathbb{R}^{1 \times d}$ is a weight matrix, and
%$b^{(r)} \in \mathbb{R}^d$ is a scalar bias.
% Similarly to that of $a$, all rows of $W^{(r)},b^{(r)}$ can be enforced to be identical as well.

%Given the attention and reset gates, we define the updated query in the current layer, ${\bf %u}^l_t$, by
%\begin{equation}\label{eqn:ut}
%    \tilde{{\bf u}}^l_t = \tanh({\bf W}^{({\bf u})}[{\bf u}^{l-1}_t; {\bf m}_t] + {\bf b}^{({\bf u})})
%\end{equation}
%\begin{equation}\label{eqn:u}
%    {\bf u}^l_t = a^l_t r^l_t \tilde{{\bf u}}^l_t + (1-a^l_t) {\bf u}^l_{t-1}
%\end{equation}
%where $\tanh$ is a hyperbolic tangent activation function (applied element-wise),
%${\bf W}^{({\bf u})} \in \mathbb{R}^{d \times 2d}$ is a weight matrix,
%${\bf b}^{({\bf u})} \in \mathbb{R}^d$ is a bias vector,
%and $[;]$ is vector concatenation operation (along the row).
%$\tilde{{\bf u}}^l_t$ can be considered as the new candidate query vector after observing ${\bf m}_t$ given the query vector from the previous layer, ${\bf u}^{l-1}_t$.
%Intuitively, the current query vector is updated to a new candidate query vector, $\tilde{{\bf u}}^l_t$, if the attention gate is high and the reset gate is high.
%If the attention gate is high but the reset gate is low, the current query vector is nullified, i.e. it becomes a zero vector.
%If the attention is low, then the query vector from previous time step is propagated to the current time step.
%${u}$ has been propagated through the time until a high attention has been observed,  \note{how about reset}.  in which case the new $\tilde{{\bf u}}$ overrides it. 
%In order to stack several layers of query-regression, which is crucial for complex reasoning, ${\bf u}^l_t$ is passed to the next layer and Equations \ref{eqn:a}, \ref{eqn:r}, \ref{eqn:u}, \ref{eqn:ut} are repeated.

%\paragraph{Answering queries.} The answer to the original question will be derived by answering the updated question at the last layer.  Let $K$ be the number of layers in the network.
%We define ${\bf h}_t$ as the updated question on the last layer (Figure~\ref{fig:model}). The formulation of ${\bf h}_t$ is similar to Equation~\ref{eqn:u} but is not affected by reset gate: 
%\begin{equation}\label{eqn:h}
%{\bf h}_t = a^K_t \tilde{{\bf u}}^K_t + (1 - a^K_t){\bf h}_{t-1}
%\end{equation}
% Now we obtain the predicted answer in a sparse vector form, $\hat{y}_t$ at time $t$ of the last layer. 
%\begin{equation}
%    \hat{{\bf y}}_t = \mathrm{softmax}({\bf W}^{({\bf y})} {\bf h}_t + {\bf b}^{({\bf y})})
%\end{equation}
%where ${\bf W}^{({\bf y})} \in \mathbb{R}^{V \times d}$ is a weight matrix for $V$-way classification of the answer, 
%and ${\bf b}^{({\bf y})}$ is a bias vector.
%Note that we do not use ${\bf m}$ in the classification stage.
%This would intuitively make sense if ${\bf h}_t$ encodes all necessary information from ${\bf m}$.
%Since we are answering the question at the end of the story, the final answer of our model is $\hat{{\bf y}} = \hat{{\bf y}}_T$.

\subsection{Extensions}\label{sec:var}
Here we introduce a few extensions of QRN, and later in our experiments, we test QRN's performance with and without each of these extensions.

\paragraph{Reset gate.} Inspired by GRU~\citep{GRU}, we found that it is useful to allow the QRN unit to reset (nullify) the candidate reduced query (i.e., ${\tilde {\bf h}}_t$) when necessary.
For this we use a \emph{reset gate} function $\beta : \mathbb{R}^d \times \mathbb{R}^d \rightarrow [0,1]$, which can be defined similarly to the update gate function:
\begin{equation}\label{eq:r}
r_t = \beta({\bf x}_t, {\bf q}_t) = \sigma({\bf W}^{(r)} ({\bf x}_t \circ {\bf q}_t) + b^{(r)})
\end{equation}
where ${\bf W}^{(r)} \in \mathbb{R}^{1 \times d}$ is a weight matrix, and $b^{(r)} \in \mathbb{R}$ is a bias term. 
Equation~\ref{eq:h} is rewritten as
\begin{equation}\label{eq:hr}
{\bf h}_t = z_t r_t {\tilde {\bf h}}_t + (1 - z_t) {\bf h}_{t-1}.
\end{equation}
Note that we do not use the reset gate in the last layer.
% The intuition of the input gate is as follows.

\paragraph{Vector gates.} As in LSTM and GRU, update and reset gates can be vectors instead of scalar values for fine-controlled gating.
For vector gates, we modify the row dimension of weights and biases in Equation~\ref{eq:z} and~\ref{eq:r} from $1$ to $d$.
Then we obtain ${\bf z}_t, {\bf r}_t \in \mathbb{R}^d$ (instead of $z_t, r_t \in \mathbb{R})$, and these can be element-wise multiplied ($\circ$) instead of being broadcasted in Equation~\ref{eq:h} and~\ref{eq:hr}.



% The number of parameters required for training QRNs is xxxx; this is significantly lower than the number of parameters in the state-of-the-art reading comprehension systems of DMN~\citep{DMNN,DMN+} and end-to-end memory networks\citep{memN2N}. In particular, DMNs use xxx parameters, and end-to-end memory networks use xxx parameters. \note{number of parameters for our model vs. dmn vs. mem net}



==> ICLR 2017 QRN/03-analysis.tex <==
% \subsection{Parallelization}\label{sec:par} 
An important advantage of QRN is that the recurrent updates in Equation~\ref{eq:h} and~\ref{eq:r}  can be computed in parallel across time. 
This is in contrast with most RNN-based models that cannot be parallelized, where computing the candidate hidden state  at time $t$ explicitly requires the previous hidden state.
In QRN, the final reduced queries (${\bf h}_t$) can be decomposed into computing over candidate reduced queries (${\tilde {\bf h}}_t$), without looking at the previous reduced query.
Here we primarily show that the query update in Equation~\ref{eq:h} can be parallelized by rewriting the equation with matrix operations. 
The extension to Equation~\ref{eq:r} is straightforward.
The proof for QRN with vector gates is shown in Appendix~\ref{sec:app-b}.
%Please see the appendix for the case when $a_t$ is a $d$-dimensional vector.
The recursive definition of Equation~\ref{eq:h} can be explicitly written as
\begin{equation}\label{eq:exp}
    {\bf h}_t 
    = \sum_{i=1}^{t} \left[\prod_{j=i+1}^{t}  1-z_j \right] z_i \tilde{{\bf h}}_i
    = \sum_{i=1}^{t} \exp \left \{\sum_{j=i+1}^{t} \log \left(1 - z_j \right) \right \}
    z_i \tilde{{\bf h}}_i.
\end{equation}
Let $b_i = \log(1-z_i)$ for brevity.
Then we can rewrite Equation~\ref{eq:exp} as the following equation:

\begin{equation}\label{eq:mat}
\begin{pmatrix}
{\bf h}_1^\top \\
{\bf h}_2^\top \\
{\bf h}_3^\top \\
\vdots \\
{\bf h}_T^\top
\end{pmatrix}
 = \left[
 \exp\left\{
 \begin{pmatrix}
 0 & -\infty & -\infty & \ldots & -\infty \\
 b_2  & 0 & -\infty & \ldots & -\infty\\
 b_2 +b_3  & b_3 & 0 & \ldots & -\infty\\
 \vdots & \vdots & \vdots & \ddots & \vdots\\
 \sum_{j=2}^T b_j & \sum_{j=3}^T b_j & \sum_{j=4}^T b_j &\ldots & 0
 \end{pmatrix}\right\}
\right]
\begin{pmatrix}
z_1 \tilde{{\bf h}}^\top_1 \\
z_2\tilde{{\bf h}}^\top_2 \\
z_3\tilde{{\bf h}}^\top_3 \\
\vdots \\
z_T\tilde{{\bf h}}^\top_T
\end{pmatrix}
\end{equation}
Let ${\bf H} = [{\bf h}_1^\top ; \ldots ; {\bf h}_T^\top]$ 
be a $T$-by-$d$ matrix where the transposes ($\top$) of the column vectors ${\bf h}_t$ are concatenated across row.
We similarly define $\tilde{{\bf H}}$ from $\tilde{{\bf h}}_t$. 
Also, let ${\bf z}=[z_1; \ldots ; z_T]$ and ${\bf b}=[0; b_2; \dots ; b_T]$ be column vectors (note that we use $0$ instead of $b_1$).
Then Equation~\ref{eq:mat} is: 
\begin{equation}\label{eq:short}
{\bf H} = \left[ {\bf L} \circ \exp \left( {\bf L}\left[{\bf B} \circ {\bf L}'\right]\right) \right]
 \left[ {\bf Z} \circ \tilde{{\bf H}} \right]
\end{equation}
where ${\bf L}, {\bf L}' \in \mathbb{R}^{T \times T}$ are lower and \emph{strictly} lower triangular matrices of $1$'s, respectively, 
$\circ$ is element-wise multiplication, and
${\bf B}$ is a matrix where $T$ ${\bf b}$'s are tiled across the column, i.e. ${\bf B} = [{\bf b}, \dots , {\bf b}] \in \mathbb{R}^{T \times T}$, 
and similarly ${\bf Z} = [{\bf z}, \dots , {\bf z}] \in \mathbb{R}^{T \times d}$. 
All implicit operations are matrix multiplications.
With reasonable $N$ (batch size), $d$ and $T$ (e.g. $ N,d,T=100$), matrix operations in Equation~\ref{eq:short} can be comfortably computed in most modern GPUs.






==> ICLR 2017 QRN/04-related.tex <==

%Kwiatkowski13scalingsemantic,bordes2014question,
%The first category of neural approaches to question answering  use neural sequence modeling to capture the dependencies between sentences in a story~\citep{RNNsearch}. However, it is difficult to capture long-term dependencies between sentences with this model.  Additionally, the architecture is quite complex and requires optimizing a large set of parameters. 

% List of things to compare
% 1. RNN, GRU, LSTM: simpler structure, parallelizable, specialized for question answering (two inputs) but possibly generalizable
% 2. Memory networks: not attention-based mechanism, simpler, RNN-based model, no summarization (cumulation) which helps preserve locality
% 2-2: Neural reasoner: some variant of memory networks with more complex update module
% 3. Dynamic memory networks: similar story
% 4. Reasoning in vector space: not an end-to-end model
% Previous solutions to question answering use open information extraction or textual semantic parsing to query or create a knowledge base~\citep{yates,scott,hosseini2014learning,berant2013semantic,tony,Seo2015SolvingGP}. 
% Here, we primarily describe the most related approaches, which perform multi-hop reasoning over a given context (either story or dialog) in an end-to-end fashion (sketched in Figure~\ref{fig:models}). In our experiments we show that QRNs outperform all these models. 
%Figure~\ref{fig:models} shows the comparison between QRN and other relevant models.

\begin{figure}[t]

\begin{subfigure}[htbp]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/qrn.pdf}
\caption{  QRN }
\label{fig:qrn}
\end{subfigure}
\begin{subfigure}[htbp]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/n2n.pdf}
\caption{ N2N~\citep{memN2N} }
\label{fig:memn2n}
\end{subfigure}
\begin{subfigure}[htbp]{0.32\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/dmn.pdf}
\caption{ DMN+~\citep{DMN+} }
\label{fig:dmn}
\end{subfigure}
\caption{\small The schematics of QRN and the two state-of-the-art models, End-to-End Memory Networks (N2N) and Improved Dynamic Memory Networks (DMN+), simplified to emphasize the differences among the models. 
AGRU is a variant of GRU where the update gate is replaced with soft attention, proposed by \citet{DMN}.
%The circle nodes are memory access controllers that summarize the entire memory in each layer and decide attention weights in the next layer.
%Note that this is necessary for MemN2N and DMN+, but not needed for QRN. 
For QRN and DMN+, only forward direction arrows are shown.}
\label{fig:models}
\end{figure}

QRN is inspired by RNN-based models with gating mechanism, such as LSTM~\citep{lstm} and GRU~\citep{GRU}.
%As QRN is designed for sequential data with query, its unit accepts two inputs (query and sentences) instead of one input. 
While GRU and LSTM use the previous hidden state and the current input to obtain the candidate hidden state, QRN only uses the current two inputs to obtain the candidate reduced query (equivalent to candidate hidden state).
We conjecture that this not only gives computational advantage via parallelization, but also makes training easier, i.e., avoiding vanishing gradient (which is critical for long-term dependency), overfitting (by simplifying the model), and converging to local minima.
%The advantage of QRN over other RNN-based models is experimentally shown in Table~\ref{tab:summary}, where LSTM performs poorly.

The idea of structurally simplifying (constraining) RNNs for learning longer-term patterns has been explored in recent previous work, such as Structurally Constrained Recurrent Network~\citep{scrn} and Strongly-Typed Recurrent Neural Network (STRNN)~\citep{strnn}. 
QRN is similar to STRNN in that both architectures use gating mechanism, and the gates and the candidate hidden states do not depend on the previous hidden states, which simplifies the recurrent relation. 
However, QRN can be distinguished from STRNN in three ways.
First, QRN’s update gate simulates attention mechanism, measuring the relevance between the input sentence and query. On the other hand, the gates in STRNN can be considered as the simplification of LSTM/GRU by removing their dependency on previous hidden state.
Second, QRN is an RNN that is natively compatible with context-based QA tasks, where the QRN unit accepts two inputs, i.e. each context sentence and query. 
This is distinct from STRNN which has only one input. 
Third, we show that QRN is timewise-parallelizable on GPUs. Our parallelization algorithm is also applicable to STRNN.

End-to-end Memory Network (N2N)~\citep{memN2N} uses external memory with multi-layer attention mechanism to focus on sentences that are relevant to the question.
There are two key differences between N2N and our  QRN. 
First, N2N summarizes the entire memory in each layer to control the attention in the next layer (circle nodes in Figure~\ref{fig:memn2n}).
Instead, QRN does not have any controller node (Figure~\ref{fig:qrn}) and is able to focus on relevant sentences through the update gate that is internally embodied within its unit.
Second, N2N adds time-dependent trainable weights to the sentence representations to model the time dependency of the sentences (as discussed in Section~\ref{sec:intro}).
QRN does not need such additional weights as its inherent RNN architecture allows QRN to effectively model the time dependency.
Neural Reasoner~\citep{NR} and Gated End-to-end Memory Network~\citep{perez2016gated}) are variants of MemN2N that share its fundamental characteristics.


Improved Dynamic Memory Network (DMN+)~\citep{DMN+} uses the hybrid of the attention mechanism and the RNN architecture to model the sequence of sentences.
It consists of two distinct GRUs, one for the time axis (rectangle nodes in Figure~\ref{fig:dmn}) and one for the layer axis (circle nodes in Figure~\ref{fig:dmn}).
Note that the update gate of the GRU for the time axis is replaced with external softmax attention weights.
DMN+ uses the time-axis GRU to summarizes the entire memory in each layer, and then the layer-axis GRU controls the attention weights in each layer.
In contrast, QRN is simply a single recurrent unit without any controller node. 



% Memory Networks~\citep{memNet} and Dynamic Memory Networks~\citep{DMN} are earlier models that inspired MemN2N and DMN+, respectively.
% However, they are strongly supervised (i.e. during training they are given what facts are relevant to the question), where QRN is only supervised by the answers to the questions. 
% So we do not make a direct comparison against them.

% While \citet{Mitra2016AddressingAQ} and \citet{RiVS} have shown near-perfect accuracies in bAbI QA dataset, they are largely rule-based (requiring human efforts), they use different models for different tasks, and/or they use external language resources such as dependency parser.
% So we do not consider them as end-to-end machine comprehension systems.


% The inherent goal in most question answering methods is to track the progression of the state of the story by either updating all the facts after each iteration or accumulating all the information through time steps and then updating the summarized information at each layer. Encoding complex inter-dependencis between facts, specially when their number  grows, imposes challenges in efficient representation and learning. The main issue with sequence modeling solutions (RNN, GRU, LSTM, RNNSearch~\citep{bahdanau2014neural}) is the complexity of these models. QRNs differ from all the previous methods in that it aims at the logical regression of the question itself and does not require complicated models  to encode complex interdependencies between facts. 

% QRNs do not accumulate information across time steps and hence is highly parrallelizable. This enables QRNs to answer to the questions at any time step and model locality. This is particularly interesting for online streaming applications where facts are observed in an streaming fashion. Finally, the intermediate states of the QRN, represented by updated questions, are interpretable offering interesting applications for debugging and  dialogue systems. 
 
% Attention mechanism have been successfully used in neural networks across a wide variety of tasks: image classification~\citep{stollenga2014deep}, image captioning~\citep{xu2015show, malinowski2014multi}, and machine translation~\citep{cho2014learning,bahdanau2014neural}. Attention and memory mechanism have also been used in solving algorithmic problems~\citep{joulin2015inferring,kaiser2015neural} and visual question answering~\citep{yang2015stacked,andreas2016learning}.%andreas2015deep %andreas2015deep %graves2014neural



%\note{Some variation of this text also will be in related work: }
%The first category (CITE) treated the story as a sequence of sentences, and used a recurrent neural network in which  each sentence occupies single cell. However, this model is not able to capture the long-term dependencies between sentences.  Additionally, the architecture is quite complex and requires optimizing a large set of parameters. 

%The second category (CITE) are designed to capture the long-term dependencies among sequential sentences through a shared memory. End-to-end memory networks (cite) use an attention mechanism that at each layer selects the relevant facts to the question and updates the memory cells at next layers. %nat each layer.  It then updates memory cells at next layers It then updates the memory cells at next layer,     attention mechanism, where at each layer, the question selects relevant facts and transforms the question to a new vector so that it can choose other facts in the next layer.
%In order to model the time dependencies between the facts, these networks define time-variant variables on the facts. 
%This model is simpler and more interpretable than the previous category, but \note{should explain why it is bad?}
%The first category can theoretically address this issue, but pure attention mechnaism cannot handle these. In order to resolve such time dependency, end to end memory networks puts time-variant variables on the facts.
%Also, they update the memory every layer, which is computationally expensive and uninterpretable. \note{Our layer also intuitively update the memory, right?}

%The third model (dynamic memory networks) combine the advantages of both networks. They incorporate recurrent neural networks both to model the time dependencies among the facts and to update the memory layers. In addition, they use an attention layer to choose relevant facts at each layer. 
%But it makes the model very complicated; there is possibility of reverse engineering the synthetic data.

%In details, what's different from DMN.
%differences:

%1. we are using sigmoid attention, where they use softmax attention -> completely changes the architecture, as we could have strong attention on several times.

%2. DMN extensively uses RNN such as GRU. It obtains the updated memory by putting a layer (Wx + b) between previous output and the current inputs.
%Ours doesn't have any RNN, just passing based on the attention. Hence:
%- Simpler model, simpler architecture
%- More interpretable
%- Can be parallelized, overcoming the limitation of RNN in general (Section~\ref{sec:par}
%3. In DMN+, in memory update, new memory depends on prev memory and context vector, which is at the end of GRU. Huge dependence on the end of vector context.
%In ours, depends on prev memory and original fact. That's it (hence parallelizable).
%% Figures %%



==> ICLR 2017 QRN/05-qa.tex <==
%%%%%%%%%%%% table & figure name %%%%%%%%%%%%
% result summary        : sumamry
% visualization summary : att-summary
% result all            : qa-all, dialog-all
% visualization all     : qa-att-all, dialog-att-all
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% add Visualization paragraph.
% TODO: result summary - combine or separate?
% TODO: match appendix?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Data}
\paragraph{bAbI story-based QA dataset} bAbI story-based QA dataset~\citep{babi} is composed of 20 different tasks (Appendix~\ref{sec:app-a}), each of which has 1,000 (1k) synthetically-generated story-question pair. 
A story can be as short as two sentences and as long as 200+ sentences.
A system is evaluated on the accuracy of  getting the correct answers to the questions. % and the authors of the dataset define that a system passes a task if its error rate is no more than $5\%$.
The answers are single words or lists (e.g. ``football, apple'').
Answering questions in each task requires selecting a set of relevant sentences and applying different kinds of logical reasoning over them. 
The dataset also includes 10k training data (for each task), which allows training more complex models. 
Note that DMN+~\citep{DMN+} only reports on the 10k dataset. 
% We also report the reproduced 1k result of DMN+ using the code from a third party\footnote{Code obtained from: \url{github.com/therne/dmn-tensorflow}}, as the authors of DMN+ do not release their code.
% Following previous work, QRN is only supervised by question answers.
% Hence we do not compare QRN against Memory Networks~\citep{memNet} and DMN~\citep{DMN}, which require strong supervision of supporting facts during training.
%We do not use these supervision (hence weakly supervised by the answer only), which aligns with recent previous work~\citep{}.
\paragraph{bAbI dialog dataset}
bAbI dialog dataset~\citep{bordes2016learning} consists of 5 different tasks (Table~\ref{tab:dialog-all}), each of which has 1k synthetically-generated goal-oriented dialogs between a user and the system in the domain of restaurant reservation. 
Each dialog is as long as 96 utterances and comes with external knowledge base (KB) providing information of each restaurant.
The authors also provide Out-Of-Vocabulary (OOV) version of the dataset, where many of the words and KB keywords in test data are not seen during training.
A system is evaluated on the accuracy of its response to each utterance of the user, choosing from up to 2500 possible candidate responses.
A system is required not only to understand the user's request but also refer to previous conversations in order to obtain the context information of the current conversation.
% Its goal is to make a conversation with an user in system's position by taking order, asking question about the request, and answering the question of an user. 
% The dataset was synthetically-generated by a simulation, and contains 5 different tasks. Each task has train set, development set, and two test sets with each 1,000 (1k) dialogs. The first test set is a plain test set and the second one contains OOV words, which are provided in KB but not provided in train set. See Table~\ref{tab:dialog-all} for the complete list of the 5 tasks.

% The sentences in dialog except the last one are considered as context, and the last sentence from an user is considered as a query. A story can be zero if it is the first sentence of the dialog, and as long as 96 sentences. Answer candidates are given and the number is 400 to 2500. In order to select correct response, the system has to understand not only requests of a user but also which request are currently valid and which information does the system additionally need to make a reservation. 

\paragraph{DSTC2 (Task 6) dialog dataset} 
~\cite{bordes2016learning} transformed the Second Dialog State Tracking Challenge (DSTC2) dataset~\citep{henderson2014second} into the same format as the bAbI dialog dataset, for the measurement of performance on a real dataset.
Each dialog can be as long as 800+ utterances, and a system needs to choose from 2407 possible candidate responses for each utterance of the user.
Note that the evaluation metric of the original DSTC2 is different from that of the transformed DSTC2, so previous work on the original DSTC2 should not be directly compared to our work.
We will refer to this transformed DSTC2 dataset by ``Task 6'' of dialog dataset.

%\sewon{
%We also test our model on the dialog dataset from The Second Dialog State Tracking Challenge\citep{henderson2014second}. It is a real dataset, and is originally for tracking state of given dialog. bAbI dialog dataset converted this dialog to the form of bAbI dialog and provides it as task 6. Note that to avoid confusion of the original DSTC2 for stack tracking and the converted DSTC2 for dialog, we call DSTC2 dataset used in this paper DSTC2 dialog dataset. Since DSTC2 dialog dataset is a real data, it is much noisier and has more various situation compared to bAbI dialog dataset. A story can be zero if it is the first sentence of the dialog, and as long as 800+ sentences. As bAbI dialog, answer candidates are given and the number is 2407.
%}

\subsection{Model Details}

\paragraph{Input Module.} %\note{this can be summarized}
In the input module, we are given sentences (previous conversations in dialog) ${\bm x}_t$ and a question (most recent user utterance) ${\bm q}$, and we want to obtain their vector representations, ${\bf x}_t, {\bf q} \in \mathbb{R}^d$.
We use a trainable embedding matrix ${\bf A} \in \mathbb{R}^{d \times V}$ to encode the one-hot vector of each word ${\bm x}_{tj}$ in each sentence ${\bm x}_t$ into a $d$-dimensional vector ${\bf x}_{tj} \in \mathbb{R}^d$.
Then the sentence representation ${\bf x}_t$ is obtained by Position Encoder~\citep{memNet}. %: ${\bf x}_t = \sum_j {\bf l}_j \circ {\bf x}_{tj}$ where $k$-th element of the vector ${\bf l}_j \in \mathbb{R}^d$ is $ (1-j/J)-(k/d)(1-2j/J)$ (assuming 1-based indexing), where $J$ is the number of words in ${\bm x}_t$.
%Note that the order of words affects ${\bf x}_t$.
The same encoder with the same embedding matrix is also used to obtain the question vector ${\bf q}$ from ${\bm q}$.

\paragraph{Output Module for story-based QA.} %\note{this can be summarized}
In the output module, we are given the vector representation of the predicted answer $\hat{\bf y}$ and we want to obtain the natural language form of the answer, $\hat{\bm y}$.
We use a $V$-way single-layer softmax classifier to map $\hat{\bf y}$ to a $V$-dimensional sparse vector, $\hat{\bf v} = \mathrm{softmax}\left( {\bf W}^{(y)} \hat{\bf y} \right) \in \mathbb{R}^V$, where ${\bf W}^{(y)} \in \mathbb{R}^{V \times d}$ is a weight matrix.
Then the final answer $\hat{\bm y}$ is simply the argmax word in $\hat{\bf v}$. 
%For 10k dataset, we instead use $\hat{\bf v} = \mathrm{softmax}\left( {\bf W}^{(y)} [\hat{\bf y};{\bf q}] \right)$ (hence ${\bf W}^{(y)} \in \mathbb{R}^{V \times 2d}$).
To handle questions with multiple-word answers, we consider each of them as a single word that contains punctuations such as space and comma, and put it in the vocabulary.

\paragraph{Output Module for dialog.}
We use a fixed number single-layer softmax classifiers, each of which is similar to that of the sotry-based QA model, to sequentially output each word of the system's response.
While it is similar in spirit to the RNN decoder~\citep{GRU}, our output module does not have a recurrent hidden state or gating mechanism.
Instead, it solely uses the final ouptut of the QRN, $\hat{\bf y}$, and the current word output to influence the prediction of the next word among possible candidates.
% We use a single-layer softmax classifier as QA model, with some modifications. 
% In bAbI diaog datasets, some answers take the same format, which are `API CALL', `What do you think of this option', and `Here it is'. The softmax classifier has answer candidates which are original sentences and $3$ special cases with same format. If one of special cases is selected, another softmax is used to select specific option. For example, in the case of `API CALL' the next softmax predicts what cuisine, location, availability and price range the system is calling. In the case of `What do you think of this option', the next softmax predicts what restaurant does the system.


%% to be moved to the appendix

\paragraph{Training.} 
We withhold $10\%$ of the training  for development.
We use the hidden state size of 50 by deafult.
Batch sizes of $32$ for bAbI story-based QA 1k, bAbI dialog and DSTC2 dialog, and $128$ for bAbI QA 10k are used.
The weights in the input and output modules are initialized with zero mean and the standard deviation  of $1/\sqrt{d}$.
Weights in the QRN unit are initialized using techniques by \citet{glorot2010understanding}, and are tied across the layers.
Forget bias of $2.5$ is used for update gates (no bias for reset gates).
L2 weight decay of $0.001$ ($0.0005$ for QA 10k) is used for all weights.
The loss function is the cross entropy between $\hat{\bf v}$ and the one-hot vector of the true answer.
The loss is minimized by stochastic gradient descent for maximally $500$ epochs, but training is early stopped if the loss on the development data does not decrease for $50$ epochs.
The learning rate is controlled by AdaGrad~\citep{duchi2011adaptive}
with the initial learning rate of $0.5$ ($0.1$ for QA 10k).
Since the model is sensitive to the weight initialization,
we repeat each training procedure 10 times (50 times for 10k) with the new random initialization of the weights and report the result on the test data with the lowest loss on the development data.

\subsection{Results.}\label{subsec:results}
We compare our model with baselines and previous state-of-the-art models on story-based and dialog tasks (Table~\ref{tab:summary}). 
These include LSTM~\citep{lstm}, End-to-end Memory Networks (N2N)~\citep{memN2N}, Dynamic Memory Networks (DMN+)~\citep{DMN+}, Gated End-to-end Memory Networks (GMemN2N)~\citep{perez2016gated}, and Differentiable Neural Computer (DNC)~\citep{graves2016hybrid}. % which is an extension of Neural turing machine (NTM)~\citep{graves2014neural}. 
% NTM attempts to simulate a computer's program procedure, such as reading and writing memories, in a differentiable manner so that they can be trained with gradient descent. These are general models, but are also evaluated on the bAbI dataset. 
%They have been also experimented on the synthetic bAbI story-based QA to learn the underlying program procedure that leads to the answer of the question.

\paragraph{Story-based QA.} Table~\ref{tab:summary}(top) reports the summary of results of our model (QRN) and previous work on bAbI QA
(task-wise results are shown in Table~\ref{tab:qa-all} in Appendix).
In 1k data, QRN's `2r' (2 layers + reset gate + $d=50$) outperforms all other models by a large margin (2.8+\%).
In 10k dataset, the average accuracy of QRN's `6r200' (6 layers + reset gate + $d=200$) model outperforms all previous models by a large margin (2.5+\%), achieving a nearly perfect score of 99.7\%.

\paragraph{Dialog.}
 Table~\ref{tab:summary}(bottom) reports the summary of the results of our model (QRN) and previous work on bAbI dialog and Task 6 dialog (task-wise results are shown in Table~\ref{tab:dialog-all} in Appendix).
As done in previous work~\citep{bordes2016learning, perez2016gated}, we also report results when we use `Match' for dialogs. `Match' is the extension to the model which additionally takes as input whether each answer candidate matches with context (more details on Appendix).  QRN outperforms  previous work by a large margin (2.0+\%) in every comparison.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}
%\begin{center}
% \begin{tabular}{c}
%%%
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l||c|c|c|c|c|c||c|c|c|c|c} 
 \hline
\multirow{3}{*}{Task} & \multicolumn{6}{|c||}{1k} & \multicolumn{5}{|c}{10k} \\
\cline{2-12}
 & \multicolumn{4}{|c|}{Previous works} & \multicolumn{2}{|c||}{QRN} & \multicolumn{4}{|c|}{Previous works} & \multicolumn{1}{|c}{QRN}\\
 \cline{2-12}
                        & LSTM  & N2N   &DMN+$^\dagger$   & GMemN2N &2r    &3r   & N2N   & DMN+      & GMemN2N & DNC &6r200 \\ 
 \hline
  \# Failed             & 20    & 10    & 16    & 10    & 7     &{\bf 5} & 3     & 1   & 3       & 2   &{\bf 0}   \\ 
 Average error rates    & 51.3  & 15.2  & 33.2  & 12.7  &{\bf 9.9}& 11.3 & 4.2   & 2.8 & 3.7     & 3.8 &{\bf 0.3} \\
 \hline \hline 
\end{tabular}
} 
%%%
\\
\resizebox{0.88\columnwidth}{!}{
\begin{tabular}{l||c|c|c|c||c|c|c} 
 \hline
\multirow{3}{*}{Task} & \multicolumn{4}{|c||}{Plain} & \multicolumn{3}{|c}{With Match} \\
\cline{2-8} & \multicolumn{2}{|c|}{Previous works} & \multicolumn{2}{|c||}{QRN} & \multicolumn{2}{|c|}{Previous works} & \multicolumn{1}{|c}{QRN} \\
\cline{2-8}
                                      & N2N & GMemN2N &2r   & 2r100    & N2N+ & GMemN2N+ & 2r+      \\ 
 \hline

bAbI dialog Average error rates       & 13.9  & 14.3  &{\bf 5.5}  & {\bf 5.5} & 6.7   & 5.4   &{\bf 1.5}  \\
bAbI dialog (OOV) Average error rates & 30.3  & 27.9  &{\bf 11.1} &{\bf 11.1} & 11.2  & 10.3  &{\bf 2.3} \\
 \hline
DSTC2 dialog Average error rates      & 58.9  & 52.6  & 49.5      & {\bf 48.9}   & 59.0  & 51.3  &{\bf 49.3}  \\ 
 
 \hline 
\end{tabular}
}
%%%
%%%
% \end{tabular}
%\end{center}

\caption{\small (top) bAbI QA dataset~\citep{babi}: number of failed tasks and average error rates (\%).
$^\dagger$ is obtained from \url{github.com/therne/dmn-tensorflow}.
(bottom) bAbI dialog and DSTC2 dialog dataset~\citep{bordes2016learning} average error rates (\%) of QRN and previous work (LSTM, N2N, DMN+, GMemN2N,  and DNC).  
For QRN, the first number (1, 2, 3) indicates the number of layers, `r' means the reset gate is used, and the last number (100, 200), if exists, indicates the dimension of the hidden state, where the default value is 50. `+' indicates that `match' (See Appendix for details) is used. The task-wise results are shown in Appendices: Table~\ref{tab:qa-all} (bAbI QA) and Table~\ref{tab:dialog-all} (dialog datasets). See Section~\ref{subsec:results} for details.}
\label{tab:summary}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Ablations.}
We test four types of ablations (also discussed in Section~\ref{sec:var}): number of layers (1, 2, 3, or 6), reset gate (r), and gate vectorization (v) and the dimension of the hidden vector (50, 100). 
We show a subset of combinations of the ablations for bAbI QA in Table~\ref{tab:summary} and Table~\ref{tab:qa-all}; other combinations performed poorly and/or did not give interesting observations.
According to the ablation results, we  infer that:
{\bf (a)} When the number of layers is only one, the model lacks reasoning capability. In the case of 1k dataset, when there are too many layers (6), it seems correctly training the model becomes increasingly difficult. In the case of 10k dataset, many layers (6) and hidden dimensions (200) helps reasoning, most notably in difficult task such as task 16.
{\bf (b)} Adding the reset gate helps.
{\bf (c)} Including vector gates hurts in 1k datasets, as the model either overfits to the training data or converges to local minima. On the other hand, vector gates in bAbI story-based QA 10k dataset sometimes help.
{\bf (d)} Increasing the dimension of the hidden state to 100 in the dialog's Task 6 (DSTC2) helps, while there is not much improvement in the dialog's Task 1-5. 
It can be hypothesized that a larger hidden state is required for real data.

% \sewon{
% We also show a subset of combinations of the ablations for bAbI dialog and DSTC2 dialog in Table~\ref{tab:dialog} and Table~\ref{tab:dialog-all}. The performance of each model does not have much differences. The model with 2 layers and 100 hidden dimension sets the state-of-art, and the model with 1 layer or the model with 50 hidden dimension lacks capability. The model with vector gate was hard to optimize and takes so much time to train.
% }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|ccc|c|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 2: Two Supporting Facts & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    Sandra picked up the apple there. & \cellcolor{red!95} 0.95 & \cellcolor{red!89}0.89 & \cellcolor{red!98}0.98 & 0.00\\
    Sandra dropped the apple. & \cellcolor{red!83}0.83 & \cellcolor{red!5} 0.05 & \cellcolor{red!92}0.92 & \cellcolor{red!1} 0.01\\
    Daniel grabbed the apple there. & \cellcolor{red!88} 0.88 & \cellcolor{red!93} 0.93 & \cellcolor{red!98} 0.98 & 0.00\\
    Sandra travelled to the bathroom. & \cellcolor{red!1} \cellcolor{red!1}0.01 & \cellcolor{red!18}0.18 & \cellcolor{red!63}0.63 & \cellcolor{red!2}0.02\\
    Daniel went to the hallway. & \cellcolor{red!1}0.01 & \cellcolor{red!24}0.24 & \cellcolor{red!62}0.62 & \cellcolor{red!83}0.83\\
    \hline
    \multicolumn{5}{|l|}{Where is the apple? \hfill hallway}\\
    \hline
    \end{tabular}
    \begin{tabular}{|l|ccc|c|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 15: Deduction & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    Mice are afraid of wolves. & \cellcolor{red!11} 0.11 & \cellcolor{red!99}0.99 & \cellcolor{red!13}0.13 & \cellcolor{red!78}0.78\\
    Gertrude is a mouse. & \cellcolor{red!77}0.77 & \cellcolor{red!99}0.99 & \cellcolor{red!96}0.96 & \cellcolor{red!00}0.00\\
    Cats are afraid of sheep. & \cellcolor{red!1}0.01 & \cellcolor{red!99}0.99 & \cellcolor{red!7}0.07 & \cellcolor{red!03}0.03\\
    Winona is a mouse. & \cellcolor{red!14}0.14 & \cellcolor{red!85}0.85 & \cellcolor{red!77}0.77 & \cellcolor{red!05}0.05\\
    Sheep are afraid of wolves. & \cellcolor{red!02}0.02 & \cellcolor{red!98}0.98 & \cellcolor{red!27}0.27 & \cellcolor{red!05}0.05\\
    \hline
    \multicolumn{5}{|l|}{What is Gertrude afraid of? \hfill wolf}\\
    \hline
    \end{tabular}
    }
    
   \resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{4.5cm}|ccc|c|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 3: Displaying options & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    
    resto-paris-expen-frech-8stars? & \cellcolor{red!0} 0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!96}0.96 & \cellcolor{red!91}0.91\\
    Do you have something else? & \cellcolor{red!41}0.41 & \cellcolor{red!99}0.99 & \cellcolor{red!00}0.00 & \cellcolor{red!00}0.00\\
   Sure let me find another option. & \cellcolor{red!100}1.00 & \cellcolor{red!0}0.00 & \cellcolor{red!0}0.00 & \cellcolor{red!12}0.12\\
    %What do you think of this option: resto-paris-expen-frech-7stars & \cellcolor{red!00}0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!96}0.96 & \cellcolor{red!91}0.91\\
    %Do you have something else. & \cellcolor{red!41}0.41 & \cellcolor{red!99}0.99 & \cellcolor{red!00}0.00 & \cellcolor{red!00}0.00\\
    %Sure let me find an other option for you. & \cellcolor{red!100}1.00 & \cellcolor{red!0}0.00 & \cellcolor{red!0}0.00 & \cellcolor{red!12}0.12\\
     resto-paris-expen-frech-5stars? & \cellcolor{red!0}0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!96}0.96 & 
    \cellcolor{red!91}0.91\\
    No this does not work for me. & \cellcolor{red!00}0.00 & \cellcolor{red!00}0.00 & \cellcolor{red!14}0.14 & \cellcolor{red!00}0.00\\
    Sure let me find an other option.  & \cellcolor{red!100}1.00 & \cellcolor{red!0}0.00 & \cellcolor{red!0}0.00 & \cellcolor{red!12}0.12\\
    
    \hline
    
    
    \multicolumn{5}{|l|}{
   \hfill What do you think of this? resto-paris-expen-french-4stars} \\
    % \multicolumn{5}{|c|}{(What do you think of this option: resto-paris-expen-french-4stars)}\\
    \hline
    \end{tabular}
    %}
    
    %\resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{6.5cm}|ccc|c|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 6: DSTC2 dialog & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    
    %What kind of food would you like? & \cellcolor{red!54} 0.54 & \cellcolor{red!17}0.17 & \cellcolor{red!54}0.54 & \cellcolor{red!21}0.21\\
    %Spanish food. & \cellcolor{red!84}0.84 & \cellcolor{red!7}0.07 & \cellcolor{red!00}0.00 & \cellcolor{red!84}0.84\\
    %I'm sorry but there is no restaurant serving danish food. & \cellcolor{red!28}0.28 & \cellcolor{red!97}0.97 & \cellcolor{red!87}0.87 & \cellcolor{red!37}0.37\\
    Spanish food. & \cellcolor{red!84}0.84 & \cellcolor{red!7}0.07 & \cellcolor{red!0}0.00 & \cellcolor{red!82}0.82\\
    You are lookng for a spanish restaurant right? & \cellcolor{red!98}0.98 & \cellcolor{red!2}0.02 & \cellcolor{red!49}0.49 & \cellcolor{red!75}0.75\\
    Yes. & \cellcolor{red!1}0.01 & \cellcolor{red!100}1.00 & \cellcolor{red!33}0.33 & \cellcolor{red!13}0.13\\
    What part of town do you have in mind? & \cellcolor{red!20}0.20 & \cellcolor{red!73}0.73 & \cellcolor{red!41}0.41 & 
    \cellcolor{red!11}0.11\\
    I don't care. & \cellcolor{red!00}0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!2}0.02 & \cellcolor{red!00}0.00\\
    What price range would you like?  & \cellcolor{red!72}0.72 & \cellcolor{red!46}0.46 & \cellcolor{red!52}0.52 & \cellcolor{red!72}0.72\\
    
    \hline
    
    \multicolumn{5}{|l|}{I don't care. \hfill API CALL spanish R-location R-price}\\
    
    \hline
    \end{tabular}
    }
    
    \caption{\small (top) bAbI QA dataset~\citep{babi} visualization of update and reset gates in QRN `2r' model (bottom two) bAbI dialog and DSTC2 dialog dataset~\citep{bordes2016learning} visualization of update and reset gates in QRN `2r' model.
    %We do not put reset gate in the last layer.
    Note that the stories can have as many as 800+ sentences; we only show part of them here. More visualizations are shown in Figure~\ref{fig:qa-att-all}~(bAbI QA) and Figure~\ref{fig:dialog-att-all}~(dialog datasets).
    }
    \label{fig:att-summary}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{Parallelization.}
We implement QRN with and without parallelization in TensorFlow~\citep{tensorflow} on a single Titan X GPU to qunaitify the computational gain of the parallelization.
For QRN without parallelization, we use the RNN library provided by TensorFlow. 
QRN with parallelization gives 6.2 times faster training and inference than QRN without parallelization on average.
We expect that the speedup can be even higher for datasets with larger context.

\paragraph{Interpretations.}
An advantage of QRN is that the intermediate query updates are interpretable.
Figure~\ref{fig:model} shows intermediate local queries (${\bf q}^k_t$) interpreted in natural language, such as ``Where is Sandra?''.
In order to obtain these, we place a decoder on the input question embedding ${\bf q}$ and add its loss for recovering the question to the classification loss (similarly to \citet{NR}).
We then use the same decoder to decode the intermediate queries.
This helps us understand the flow of information in the networks. 
In Figure~\ref{fig:model}, the question \texttt{Where is apple?} is transformed into \texttt{Where is Sandra?} at $t=1$.
At $t=2$, as \texttt{Sandra dropped the apple}, the apple is no more relevant to Sandra.
We obtain \texttt{Where is Daniel?} at time $t = 3$, and it is propagated until $t=5$, where we observe a sentence (fact) that can be used to answer the query.
%In this case, the reduction function ${\bm \pho}$ is trained so that it outputs the answer to the query (``garden'') instead of another regressed query.

\paragraph{Visualization.}
Figure~\ref{fig:att-summary} shows vizualization of the (scalar) magnitudes of update and reset gates on story sentences and dialog utterances.
More visualizations are shown in Appendices: Figure~\ref{fig:qa-att-all} and Figure~\ref{fig:dialog-att-all}.
In Figure~\ref{fig:att-summary}, we observe high values on facts that provide information to answer question (the system's next utterance for dialog).
In QA Task 2 example (top left), we observe high update gate values  in the first layer on facts that state who has the \texttt{apple}, and in the second layer, the high update gate values are on those that inform where that person went to. We also observe that the forward reset gate at $t=2$ in the first layer ($\overrightarrow{r}^1_2$) is low, which is signifying that \texttt{apple} no more belongs to \texttt{Sandra}. %In QA Task 15 example(top right): we see high values of first layer on ``Gertrude is a mouse'' and high value of second layer on `Mice are afraid of wolves''.
In dialog Task 3~(bottom left), the model is able to infer that three restaurants are already recommended so that it can recommend another one. In dialog Task 6~(bottom), the model focuses on the sentences containing \texttt{Spanish}, and does not concentrate much on other facts such as \texttt{I don't care}.


==> ICLR 2017 QRN/06-sent.tex <==

\subsection{Data}
We also report QRN's performance on Stanford Sentiment Treebank~\citep{socher2013recursive}, a popular dataset for sentiment classification.
We train and test our QRN model on the binary classification task, which consists of 6920 training, 872 development, and 1820 test examples.

\subsection{Model Details}
\paragraph{Input and Output Module.} 
In sentiment analysis, there is only one sentence (instead of multiple facts in a story) and there is no explicit question.
We instead let each word of the sentence occupy single fact slot ${\bf x}_t$ in QRN, and fix the question vector ${\bf q}$ to be a constant vector of $0.1$. MemNNs
The embedding of each word is obtained via GloVe~\citep{pennington2014glove}, pre-trained on 840B Common Crawl corpora (we did not finetune).
This gives us a $300$-dimensional vector for each word.
Single $\tanh$ perceptron layer is used to transform each word vector to the QRN's hidden state size, $d$.
For output module, we use a binary single layer softmax classifier to map $\hat{y}$ to $\{positive, negative\}$ labels.

\paragraph{Training.}
Hidden state size ($d$) is set to 100 and the batch size is $128$.
We stack two layers of QRNs.
All weights are initialized using techniques from~\citet{glorot2010understanding}.
Forget bias is $2.5$  for update gates ($z^k_t$), and L2 weight decay of $0.001$ is used for all weights.
In addition, we use dropout~\citep{srivastava2014dropout} on the inputs of Equation~\ref{eq:h}.
The model is trained with AdaGrad~\citep{duchi2011adaptive} with initial learning rate of $0.5$, for 50 epochs.
We repeated the training procedure with new random weight initialization for 30 times and reported the test data result with the lowest development data loss.

\subsection{Results.}
Figure~\ref{fig:sst} shows QRN results compared against state-of-the-art methods.
% It is important to note that all of the baselines is RNN- or CNN-based architecture, while ours does not use either of those.
The result first confirms that our model can effectively incorporate inter-word dependencies without putting perceptron layers across the time axis, as QRN outperforms two strong RNN-based baselines, MV-RNN and RNTN~\citep{socher2013recursive}.
However, QRN is still short of recent state-of-the-art results, including DMN. To an extent, this is not a surprising result since inter-dependency between words is much higher than that between sentences.
In particular,  QRN is targeted for weak, long-term interdependent data; we cannot take the full advantage of QRN  in this dataset. On the other hand, 
QRN is simpler than the baseline models and can be parallelized across time. 

%As a future direction, we plan to explore combining RNN architecture with our model, though this would sacrifice the parallelization.


\begin{figure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|ccccc|c|}
\hline
& MV-RNN~\citep{socher2013recursive} & RNTN~\citep{socher2013recursive} & DCNN~\citep{DCNN} & CNN-MC~\citep{CNN-MC} & DMN~\citep{DMN} & QRN \\
\hline
Accuracy ($\%$) & 82.9 & 85.4 & 86.8 & 88.1 & 88.6 & 85.8 \\
\hline
\end{tabular}
}
\end{center}
\caption{Results on binary sentiment classification of Stanford Sentiment Treebank~\citep{socher2013recursive}}
\label{fig:sst}
\end{figure}

==> ICLR 2017 QRN/07-app-a.tex <==
Here we provide detailed per-task breakdown of our results in QA(Table~\ref{tab:qa-all}) and dialog datasets (Table~\ref{tab:dialog-all}).  
\\  


\begin{table}[ht]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|} 
 \hline
\multirow{3}{*}{Task} & \multicolumn{10}{|c||}{1k} & \multicolumn{7}{|c|}{10k} \\
\cline{2-18}
 & \multicolumn{4}{|c|}{Previous works} & \multicolumn{6}{|c||}{QRN} & \multicolumn{3}{|c|}{Previous works} & \multicolumn{4}{|c|}{QRN}\\
 \cline{2-18}
                                & LSTM  & N2N   &DMN+   &GMemN2N    & 1r   & 2    & 2r   & 3r   & 6r   & 6r200* & N2N   & DMN+  &GMemN2N & 2r   & 2rv  & 3r & 6r200\\ 
 \hline\textbf{}
 1: Single supporting fact      & 50.0  & 0.1   & 1.3   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   &13.1   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\ 
 2: Two supporting facts        & 80.0  & 18.8  & 72.3  & 8.1   & 65.7  & 1.2   & 0.7   & 0.5   & 1.5   &15.3   & 0.3   & 0.3   & 0.0   & 0.4   & 0.8   & 0.4    &0.0\\
 3: Three supporting facts      & 80.0  & 31.7  & 73.3  & 38.7  & 68.2  & 17.5  & 5.7   & 1.2   & 15.3  &13.8   & 2.1   & 1.1   & 4.5   & 0.4   & 1.4   & 0.0    &0.0\\
 4: Two arg relations           & 39.0  & 17.5  & 26.9  & 0.4   & 0.0   & 0.0   & 0.0   & 0.7   & 9.0   &13.6   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 5: Three arg relations         & 30.0  & 12.9  & 25.6  & 1.0   & 1.0   & 1.1   & 1.1   & 1.2   & 1.3   &12.5   & 0.8   & 0.5   & 0.2   & 0.5   & 0.2   & 0.3    &0.0\\ 
 6: Yes/no questions            & 52.0  & 2.0   & 28.5  & 8.4   & 0.1   & 0.0   & 0.9   & 1.2   & 50.6  &15.5   & 0.1   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 7: Counting                    & 51.0  & 10.1  & 21.9  & 17.8  & 10.9  & 11.1  & 9.6   & 9.4   & 13.1  &15.3   & 2.0   & 2.4   & 1.8   & 1.0   & 0.7   & 0.7    &0.0\\
 8: Lists/sets                  & 55.0  & 6.1   & 21.9  & 12.5  & 6.8   & 5.7   & 5.6   & 3.7   & 7.8   &15.1   & 0.9   & 0.0   & 0.3   & 1.4   & 0.6   & 0.8    &0.4\\
9 : Simple negation            & 36.0  & 1.5   & 42.9  & 10.7  & 0.0   & 0.6   & 0.0   & 0.0   & 32.7   &13.0   & 0.3   & 0.0    & 0.0   & 0.0   & 0.0   & 0.0     &0.0\\
10: Indefinite knowledge       & 56.0  & 2.6   & 23.1  & 16.5  & 0.8   & 0.6   & 0.0   & 0.0   & 3.5    &12.9   & 0.0   & 0.0    & 0.2   & 0.0   & 0.0   & 0.0     &0.0\\
 11: Basic coreference          & 38.0  & 3.3   & 4.3   & 0.0   & 11.3  & 0.5   & 0.0   & 0.0   & 0.9   &14.7   & 0.1   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 12: Conjunction                & 26.0  & 0.0   & 3.5   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   &15.1   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 13: Compound coreference       & 6.0   & 0.5   & 7.8   & 0.0   & 5.3   & 5.5   & 0.0   & 0.3   & 8.9   &13.7   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 14: Time reasoning             & 73.0  & 2.0   & 61.9  & 1.2   & 20.2  & 1.3   & 0.8   & 3.8   & 18.2  &14.5   & 0.1   & 0.0   & 0.0   & 0.2   & 0.0   & 0.0    &0.1\\
 15: Basic deduction            & 79.0  & 1.8   & 47.6  & 0.0   & 39.4  & 0.0   & 0.0   & 0.0   & 0.1   &14.7   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 16: Basic induction            & 77.0  & 51.0  & 54.4  & 0.1   & 50.6  & 54.8  & 53.0  & 53.4  & 53.5  &15.5   & 51.8  & 45.3  & 0.0   & 49.4  & 50.4  & 49.1   &0.0\\
 17: Positional reasoning       & 49.0  & 42.6  & 44.1  & 41.7  & 40.6  & 36.5  & 34.4  & 51.8  & 52.0  &13.0   & 18.6  & 4.2   & 27.8  & 0.9   & 0.0   & 5.8    &4.1\\
 18: Size reasoning             & 48.0  & 9.2   & 9.1   & 9.2   & 8.2   & 8.6   & 7.9   & 8.8   & 47.5  &14.9   & 5.3   & 2.1   & 8.5   & 1.6   & 8.4   & 1.8    &0.7\\
 19: Path finding               & 92.0  & 90.6  & 90.8  & 88.5  & 88.8  & 89.8  & 78.7  & 90.7  & 88.6  &13.6   & 2.3   & 0.0   & 31.0  & 36.1  & 1.0   & 27.9   &0.1\\
 20: Agents motivations         & 9.0   & 0.2   & 2.2   & 0.0   & 0.0   & 0.0   & 0.2   & 0.3   & 5.5   &14.6   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0   & 0.0    &0.0\\
 \hline
 \# Failed                      & 20    & 10    & 16    & 10    & 12    & 8     & 7     &{\bf 5}& 13    &20   & 3     &  1     & 3   & 2     & 2     & 3   &{\bf 0}\\ 
 Average error rates (\%)       & 51.3  & 15.2  & 33.2  & 12.7  & 20.1  & 11.7  &{\bf 9.9}& 11.3  & 20.5  &14.2 & 4.2   & 2.8  & 3.7    & 4.6   & 3.2   & 4.3    &{\bf 0.3}\\
 \hline
\end{tabular}
}
\end{center}
\caption{\small bAbI QA dataset~\citep{babi} error rates (\%) of QRN and previous work: LSTM~\citep{babi}, End-to-end Memory Networks (N2N)~\citep{memN2N}, Dynamic Memory Networks (DMN+)~\citep{DMN+}, Gated End-to-end Memory Networks(GMemN2N)~\citep{perez2016gated}. Results within each task of Differentiable Neural Computer(DNC) were not provided in its paper~\citet{graves2016hybrid}). For QRN, a number in the front (1, 2, 3, 6) indicates the number of layers. A number in the back (200) indicates the dimension of hidden vector, while the default value is 50. `r' indicates that the reset gate is used, and `v' indicates that the gates were vectorized. `*' indicates joint training.}
\label{tab:qa-all}
\end{table}



\begin{table}[ht]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l||c|c|c|c|c|c||c|c|c|} 
 \hline
\multirow{3}{*}{Task} & \multicolumn{6}{|c||}{Plain} & \multicolumn{3}{|c|}{With Match} \\
\cline{2-10} & \multicolumn{2}{|c|}{Previous works} & \multicolumn{4}{|c||}{QRN} & \multicolumn{2}{|c|}{Previous works} & \multicolumn{1}{|c|}{QRN} \\
 \cline{2-10}
                                & N2N    & GMemN2N   &1r  &2r   & 2r100 &2rv  & N2N+  & GMemN2N+ & 2r+      \\ 
 \hline
  1: Issuing API calls           & 0.1   &{\bf 0.0}   & 0.02  & {\bf 0.0}   & {\bf 0.0}   & {\bf 0.0}   & {\bf 0.0}   & {\bf 0.0}   & {\bf 0.0}     \\ 
 2: Updating API calls          & {\bf 0.0}   & {\bf 0.0}   & 0.11  & 0.01  & {\bf 0.0}   & {\bf 0.0}   & 1.7   &{\bf 0.0}   &{\bf 0.0}  \\
 3: Displaying options          & 25.1  & 25.1  & {\bf 12.6}  & {\bf 12.6} & {\bf 12.6} &{\bf 12.6}  & 25.1 & 25.1  &{\bf 7.6}   \\
 4: Providing extra information & 40.5  & 42.8  &{\bf 14.3}  & {\bf 14.3} &{\bf 14.3} &{\bf 14.3}  &{\bf 0.0}  &{\bf 0.0}   &{\bf 0.0}    \\
 5: Conducting full dialogs     & 3.9   & 3.7   & 9.4  &{\bf 0.6}  & 0.7  & 0.9  & 6.6   & 2.0   &{\bf 0.0}     \\ 
 \hline
 Average error rates (\%)            & 13.9  & 14.3  & 7.3  & {\bf 5.5}     &{\bf 5.5}       & 5.6      & 6.7   & 5.4   &{\bf 1.5}  \\
 \hline
 \hline
 1 (OOV): Issuing API calls             & 27.7  & 17.6  &{\bf 6.6}  & {\bf 6.6}  &{\bf 6.6}  & {\bf 6.6}  & 3.5   &{\bf 0.0}   &{\bf 0.0}   \\
 2 (OOV): Updating API calls            & 21.1  & 21.1  & 8.5  & 8.4  &{\bf 8.4}   & 8.5  & 5.5   & 5.8   &{\bf 0.0 } \\
 3 (OOV): Displaying options            & 25.6  & 24.7  &{\bf 12.4}  & {\bf 12.4} &{\bf 12.4} & 12.5 & 24.8  & 24.9  &{\bf 7.7}  \\
 4 (OOV): Providing extra information   & 42.4  & 43.0  &{\bf 14.3}  &{\bf 14.3} & 14.4 &14.4  &{\bf 0.0}  &{\bf 0.0}   &{\bf 0.0} \\
 5 (OOV): Conducting full dialogs       & 34.5  & 33.3  & 19.5  & 14.0 & 13.71 &{\bf 13.6} & 22.3  & 20.6  &{\bf 4.0}   \\ 
 \hline
 Average error rates (\%)                    & 30.3  & 27.9  & 12.3 & {\bf 11.1} & {\bf 11.1} &{\bf 11.1}  & 11.2  & 10.3  &{\bf 2.3} \\
 \hline
 \hline
 6: DSTC2 dialog                        & 58.9 & 52.6 & 49.9 & 49.5  &{\bf 48.9}  & 53.8  & 59.0  & 51.3  &{\bf 49.3}  \\
 \hline 
\end{tabular}
}
\end{center}
\caption{ \small bAbI dialog and DSTC2 dialog dataset~\citep{bordes2016learning} average error rates (\%) of QRN and previous work: End-to-end Memory Networks(N2N~\citep{bordes2016learning}) and Gated End-to-end Memory Networks(GMemN2N~\citep{perez2016gated}). For QRN, a number in the front (1, 2, 3, 6) indicates the number of layers and a number in the back (100) indicates the dimension of hidden vector, while the default value is 50. `r' indicates that the reset gate is used, `v' indicates that the gates were vectorized, and `+' indicates that `match' was used. }
\label{tab:dialog-all}
\end{table}











==> ICLR 2017 QRN/08-app-b.tex <==

For vector gates, we have ${\bf z}_t \in \mathbb{R}^d$ instead of $z_t \in \mathbb{R}$. Therefore the following equation replaces Equation~\ref{eq:exp}:


\begin{equation}\label{eq:v-exp}
    {\bf h}_t 
    = \sum_{i=1}^{t} \exp \left \{
    \begin{pmatrix}
    \sum_{j=i+1}^{t} \log \left(1 - {z_j}^1 \right) \\
    \sum_{j=i+1}^{t} \log \left(1 - {z_j}^2 \right) \\
    \vdots \\
    \sum_{j=i+1}^{t} \log \left(1 - {z_j}^d \right)
    \end{pmatrix}
    \right
    \} \circ
    {\bf z}_i \circ
    \tilde{{\bf h}}_i
\end{equation}

where ${z_j}^k$ is the $k$-th column vector of ${z_j}$.
Let $b_{ij} = \log(1-{z_i}^j) $ for brevity.
\begin{comment}
and let ${\bf B_{j}} $ as following :
\begin{equation}\label{eq:v-b}
    {\bf B_j} =
    \begin{pmatrix}
        0 & -\infty & -\infty & \ldots & -\infty \\
        b_{2j}  & 0 & -\infty & \ldots & -\infty\\
        b_{2j} + b_{3j}  & b_{3j} & 0 & \ldots & -\infty\\
        \vdots & \vdots & \vdots & \ddots & \vdots\\
        \sum_{k=2}^T b_{kj} & \sum_{k=3}^T b_{kj} & \sum_{k=4}^T b_{kj} &\ldots & 0
    \end{pmatrix}
\end{equation}
\end{comment}
Then, we can rewrite Equation~\ref{eq:mat} as following:

\begin{comment}
\begin{equation}\label{eq:v-mat}
\begin{pmatrix}
{\bf h}_1^\top \\
{\bf h}_2^\top \\
{\bf h}_3^\top \\
\vdots \\
{\bf h}_T^\top
\end{pmatrix}
 = \left[
 \exp\left\{
 \begin{pmatrix}
    {\bf B_1} \\
    {\bf B_2} \\
    \vdots \\
    {\bf B_d}
 \end{pmatrix}\right\}
\right]
\begin{pmatrix}
{\bf z}_1 \circ \tilde{{\bf h}}^\top_1 \\
{\bf z}_2 \circ \tilde{{\bf h}}^\top_2 \\
{\bf z}_3 \circ \tilde{{\bf h}}^\top_3 \\
\vdots \\
{\bf z}_T \circ \tilde{{\bf h}}^\top_T
\end{pmatrix}
\end{equation}

Here, implicit operation is $3D$-matrix multiplications. It takes a $T$-by-$T$-by-$d$ matrix and a $T$-by-$d$ matrix and takes matrix multiplication of a $T$-by-$T$ matrix and a $T$ vector  in element-wise on $d$ dimension, and has a $T$-by-$d$ matrix as output i.e.

\end{comment}

\begin{equation}\label{eq:v-mat}
{\begin{pmatrix}
{\bf h}_1^\top \\
{\bf h}_2^\top \\
{\bf h}_3^\top \\
\vdots \\
{\bf h}_T^\top
\end{pmatrix}}^j
 = \left[
 \exp\left\{
    \begin{pmatrix}
        0 & -\infty & -\infty & \ldots & -\infty \\
        b_{2j}  & 0 & -\infty & \ldots & -\infty\\
        b_{2j} + b_{3j}  & b_{3j} & 0 & \ldots & -\infty\\
        \vdots & \vdots & \vdots & \ddots & \vdots\\
        \sum_{k=2}^T b_{kj} & \sum_{k=3}^T b_{kj} & \sum_{k=4}^T b_{kj} &\ldots & 0
    \end{pmatrix}
\right\}
\right]
{\begin{pmatrix}
{\bf z}_1 \circ \tilde{{\bf h}}^\top_1 \\
{\bf z}_2 \circ \tilde{{\bf h}}^\top_2 \\
{\bf z}_3 \circ \tilde{{\bf h}}^\top_3 \\
\vdots \\
{\bf z}_T \circ \tilde{{\bf h}}^\top_T
\end{pmatrix}}^j
\end{equation}


Let ${\bf H} = [{\bf h}_1^\top ; \ldots ; {\bf h}_T^\top]$ 
be a $T$-by-$d$ matrix where the transposes ($\top$) of the column vectors ${\bf h}_t$ are concatenated across row.
We similarly define $\tilde{{\bf H}}$ from $\tilde{{\bf h}}_t$. 
Also, let ${\bf z}=[z_1; \ldots ; z_T]$, and ${\bf B}_d$ be a $T$-by-$T$ matrix where $T$ $[0; b_{2d}; \dots ; b_{Td}]$'s are tiled across the column.

Then Equation~\ref{eq:v-mat} is: 

\begin{equation}\label{eq:v-short}
{\bf H} = \begin{pmatrix}
    \left[ {\bf L} \circ \exp \left( {\bf L}\left[{\bf B}_1 \circ {\bf L}'\right]\right)\right]
        \left[ {\bf Z} \circ \tilde{{\bf H}} \right]^1\\
    \left[ {\bf L} \circ \exp \left( {\bf L}\left[{\bf B}_2 \circ {\bf L}'\right]\right)\right]
        \left[ {\bf Z} \circ \tilde{{\bf H}} \right]^2\\
    \vdots \\
    \left[ {\bf L} \circ \exp \left( {\bf L}\left[{\bf B}_d \circ {\bf L}'\right]\right)\right]
        \left[ {\bf Z} \circ \tilde{{\bf H}} \right]^d
 \end{pmatrix} 
\end{equation}

where ${\bf L}, {\bf L}' \in \mathbb{R}^{T \times T} $ are lower and \emph{strictly} lower triangular matrices of $1$'s are tiled across the column. ${\bf Z} = [{\bf z}_1, \dots , {\bf z}_d] \in \mathbb{R}^{T \times d}$. 


==> ICLR 2017 QRN/09-app-c.tex <==


\paragraph{Visualization of Story-based QA.}
Figure~\ref{fig:qa-att-all} shows visualization of models for story-based QA tasks.

In the task 3 (left), the model focuses on the facts that contain 'football' in the first layer, and found out where Mary journeyed to before the bathroom in the second layer. In task 7 (right), the model focuses on the facts that provide information about  the location of Sandra.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|ccc|c|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 3: Three Supporting Facts & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    Mary got the football there. & \cellcolor{red!82} 0.82 & \cellcolor{red!100}1.00 & \cellcolor{red!0}0.0 & \cellcolor{red!6}0.06\\
    John went back to the bedroom. & \cellcolor{red!1}0.01 & \cellcolor{red!00}0.00 & \cellcolor{red!72}0.72 & \cellcolor{red!57}0.57\\
    Mary journeyed to the office. & \cellcolor{red!1}0.01 & \cellcolor{red!04}0.04 & \cellcolor{red!6}0.06 & \cellcolor{red!88}0.88\\
    Mary journeyed to the bathroom. & \cellcolor{red!44}0.44 & \cellcolor{red!00}0.00 & \cellcolor{red!89}0.89 & \cellcolor{red!05}0.05\\
    Mary dropped the football. & \cellcolor{red!62}0.62 & \cellcolor{red!1}0.01 & \cellcolor{red!00}0.00 & \cellcolor{red!03}0.03\\
    \hline
    \multicolumn{5}{|l|}{Where was the football before the bathroom? \hfill office}\\
    \hline
    \end{tabular}
    \begin{tabular}{|c|ccc|c|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 7: Counting & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    Mary journeyed to the garden. & \cellcolor{red!67} 0.67 & \cellcolor{red!8}0.08 & \cellcolor{red!58}0.58 & \cellcolor{red!12}0.12\\
    Mary journeyed to the office. & \cellcolor{red!91}0.91 & \cellcolor{red!44}0.44 & \cellcolor{red!11}0.11 & \cellcolor{red!21}0.21\\
    Sandra grabbed the apple there. & \cellcolor{red!2}0.02 & \cellcolor{red!34}0.34 & \cellcolor{red!92}0.92 & \cellcolor{red!89}0.89\\
    Sandra discarded the apple. & \cellcolor{red!26}0.26 & \cellcolor{red!61}0.61 & \cellcolor{red!95}0.95 & \cellcolor{red!97}0.97\\
    Daniel went to the bedroom. & \cellcolor{red!70}0.70 & \cellcolor{red!44}0.44 & \cellcolor{red!99}0.99 & \cellcolor{red!3}0.03\\
    \hline
    \multicolumn{5}{|l|}{How many objects is Sandra carrying? \hfill none}\\
    \hline
    \end{tabular}
    }
    \caption{ Visualization of update and reset gates in QRN `2r' model for on several tasks of bAbI QA (Table~\ref{tab:qa-all}).
    We do not put reset gate in the last layer.
    Note that we only show some of recent sentences here, though the stories can have as many as 200+ sentences.
    }
    \label{fig:qa-att-all}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\paragraph{Visualization of Dialog.}
Figure~\ref{fig:dialog-att-all} shows visualization of models for dialog tasks.

In the first dialog of task 1, the model focuses on the user utterance that mentions the user's desired cuisine and location, and the current query (user's last utterance) informs the system of the number of people, so the system is able to learn that it now needs to ask the user about the desired price range. 
In the second dialog of task 1, the model focuses on the facts that provide information about the requests of the user.
In task 4 (third), the model focuses on what restaurant a user is talking about and the information about the restaurant.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{-4cm}
\begin{figure*}[t]
    \centering
    
    \resizebox{\columnwidth}{!}{\footnotesize
    \begin{tabular}{|C{11cm}|C{0.6cm}C{0.6cm}C{0.6cm}|C{1cm}|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & {Layer 2}\\
    \hline
    Task 1 Issuing API calls& $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    Good morning. & \cellcolor{red!12}0.12 & \cellcolor{red!34}0.34 & \cellcolor{red!98}0.98 & \cellcolor{red!20}0.20\\
    Hello what can i help you with today. & \cellcolor{red!97}0.97 & \cellcolor{red!97}0.97 & \cellcolor{red!12}0.12 & \cellcolor{red!12}0.12\\
    Can you book a table in rome with italian cuisine. & \cellcolor{red!0}0.00 & \cellcolor{red!87}0.87 & \cellcolor{red!100}1.00 & \cellcolor{red!100}1.00\\
    I'm on it. & \cellcolor{red!73}0.73 & \cellcolor{red!97}0.97 & \cellcolor{red!38}0.38 & \cellcolor{red!0}0.00\\
    How many people would you in your party. & \cellcolor{red!100}1.00 & \cellcolor{red!100}1.00 & \cellcolor{red!00}0.00 & \cellcolor{red!41}0.41\\
    \hline
    \multicolumn{5}{|l|}{For four people please. \hfill Which price range are you looking for.}\\
    \hline
    \end{tabular}
    }
    
    %\resizebox{\columnwidth}{!}{
    %\begin{tabular}{|c|ccc|c|}
    %\hline
    %& \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    %\hline
    %Task 6 DSTC2 dialog& $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    %\hline
    %rajmahal R-location east & \cellcolor{red!0} 0.00 & \cellcolor{red!99}0.99 & \cellcolor{red!94}0.94 & \cellcolor{red!98}0.98\\
    %rajmahal R-rating 10 & \cellcolor{red!00}0.00 & \cellcolor{red!12} 0.12 & \cellcolor{red!3}0.03 & \cellcolor{red!100} 1.00\\
    %curry-prince R-location east & \cellcolor{red!2} 0.02 & \cellcolor{red!91} 0.91 & \cellcolor{red!100} 1.00 & \cellcolor{red!00} 0.00\\
    %curry-prince R-rating 3 & \cellcolor{red!96}0.96 & \cellcolor{red!0}0.00 & \cellcolor{red!07}0.07 & \cellcolor{red!50}0.50\\
    %\hline
    %\multicolumn{5}{|l|}{For four people please \hfill rajmahal is a nice place in the east of town and the prices are moderate.} \\
    %\hline
    %\end{tabular}
    %}
    
    \resizebox{\columnwidth}{!}{\footnotesize
    \begin{tabular}{|C{11cm}|C{0.6cm}C{0.6cm}C{0.6cm}|C{1cm}|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    Task 1 Issuing API calls & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    \hline
    Can you make a restaurant reservation for eight in a cheap price range in madrid & \cellcolor{red!0}0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!93}0.93 & \cellcolor{red!100}1.00\\
    I'm on it. & \cellcolor{red!0}0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!74}0.74 & \cellcolor{red!0}0.00\\
    Any preference on a type of cuisine. & \cellcolor{red!0}0.00 & \cellcolor{red!11}0.11 & \cellcolor{red!100}1.00 & \cellcolor{red!1}0.01\\
    I love british food. & \cellcolor{red!0}0.00 & \cellcolor{red!99}0.99 & \cellcolor{red!99}0.99 & \cellcolor{red!57}0.57\\
    Okay let me look into some options for you. & \cellcolor{red!100}1.00 & \cellcolor{red!0}0.00 & \cellcolor{red!00}0.00 & \cellcolor{red!2}0.02\\ 
    \hline
    \multicolumn{5}{|l|}{<SILENCE> \hfill API CALL british madrid eight cheap}\\
    \hline
    \end{tabular}
    }

    
    
    \resizebox{\columnwidth}{!}{\footnotesize
    \begin{tabular}{|C{11cm}|C{0.6cm}C{0.6cm}C{0.6cm}|C{1cm}|}
    \hline
    & \multicolumn{3}{|c|}{Layer 1} & Layer 2\\
    \hline
    
    Task 4 Providing extra-information  & $z^1$ & $\overrightarrow{r}^1$ & $\overleftarrow{r}^1$ & $z^2$\\
    
    \hline
    
    resto-paris-expen-spanish-8stars R-phone resto-paris-expen-spanish-8stars-phone & \cellcolor{red!71}0.71 & \cellcolor{red!84}0.84 & \cellcolor{red!99}0.99 & \cellcolor{red!36}0.36\\
    
    resto-paris-expen-spanish-8stars R-address resto-paris-expen-spanish-8stars-address & \cellcolor{red!100}1.00 & \cellcolor{red!99}0.99 & \cellcolor{red!100}1.00 & 
    \cellcolor{red!100}1.00\\
    
    resto-paris-expen-spanish-8stars R-location paris & \cellcolor{red!5}0.05 & \cellcolor{red!1}0.01 & \cellcolor{red!100}1.00 & \cellcolor{red!00}0.00\\
    
    resto-paris-expen-spanish-8stars R-number four & \cellcolor{red!2}0.02 & \cellcolor{red!95}0.95 & \cellcolor{red!97}0.97 & \cellcolor{red!0}0.00\\
    
    resto-paris-expen-spanish-8stars R-price expensive & \cellcolor{red!0}0.00 & \cellcolor{red!5}0.05 & \cellcolor{red!92}0.92 & \cellcolor{red!00}0.00\\
    
    resto-paris-expen-spanish-8stars R-rating 8 & \cellcolor{red!38}0.38 & \cellcolor{red!91}0.91 & \cellcolor{red!100}1.00 & 
    \cellcolor{red!10}0.10\\
    
    What do you think of this option: resto-paris-expen-spanish-8stars & \cellcolor{red!90}0.90 & \cellcolor{red!93}0.93 & \cellcolor{red!99}0.99 & \cellcolor{red!100}1.00\\
    
    Let's do it. & \cellcolor{red!0}0.00 & \cellcolor{red!0}0.00 & \cellcolor{red!100}1.00 & \cellcolor{red!0}0.00\\
    
    Great let me do the reservation. & \cellcolor{red!98}0.98 & \cellcolor{red!99}0.99 & \cellcolor{red!97}0.97 & \cellcolor{red!0}0.00\\
    
    \hline
    
    \multicolumn{5}{|l|}{Do you have its address. \hfill Here it is: resto-paris-expen-spanish-8stars-address} \\
   %\multicolumn{5}{|c|}{(Here it is: resto-paris-expen-spanish-8stars-address)}\\

    \hline
    \end{tabular}
    }
    
    \caption{\small Visualization of update and reset gates in QRN `2r' model for on several tasks of bAbI dialog and DSTC2 dialog (Table~\ref{tab:dialog-all}).
    We do not put reset gate in the last layer.
    Note that we only show some of recent sentences here, even the dialog has more sentences.
    }
    \label{fig:dialog-att-all}
\end{figure*}



==> ICLR 2017 QRN/10-app-d.tex <==

\paragraph{Match.}
While similar in spirit, our `Match' model is slightly different from previous work~\citep{bordes2016learning, perez2016gated}. 
We use answer candidate embedding matrix, and add 2 dimension of 0-1 matrix which expresses whether the answer candidate matches with any word in the paragraph and the question. In other words, the softmax is computed by
$\hat{\bf v} = \mathrm{softmax}\left( {\bf W} [{\bf W}^{(y)};{\bf M}^{(y)}] \hat{\bf y} \right) \in \mathbb{R}^V$, where ${\bf W} \in \mathbb{R}^{d \times d}$ and ${\bf W}^{(y)} \in \mathbb{R}^{V \times (d-2)}$ are trainable weight matrices, and ${\bf M}^{(y)}\in \mathbb{R}^{V \times 2} $ is the 0-1 match matrix.



